SumREN: Summarizing Reported Speech about Events in News

A primary objective of news articles is to establish the factual record for an event, frequently achieved by conveying both the details of the specified event (i.e., the 5 Ws; Who, What, Where, When and Why regarding the event) and how people reacted to it (i.e., reported statements). However, existing work on news summarization almost exclusively focuses on the event details. In this work, we propose the novel task of summarizing the reactions of different speakers, as expressed by their reported statements, to a given event. To this end, we create a new multi-document summarization benchmark, SUMREN, comprising 745 summaries of reported statements from various public figures obtained from 633 news articles discussing 132 events. We propose an automatic silver training data generation approach for our task, which helps smaller models like BART achieve GPT-3 level performance on this task. Finally, we introduce a pipeline-based framework for summarizing reported speech, which we empirically show to generate summaries that are more abstractive and factual than baseline query-focused summarization approaches.

==> camera_ready_sections/abstract.tex <==
%\revanth{Re-wrote abstract, please take a look.}
%News articles provide various types of information, including details of the events that have happened and how people have reacted to them. Previous work on news summarization mainly tackled summarizing the event details themselves not the reactions to these events. %Reported statements within news convey important information about the reactions to these events. 
A primary objective of news articles is to establish the factual record for an event, frequently achieved by conveying both the details of the specified event (i.e., the 5 Ws; Who, What, Where, When and Why regarding the event) and how people reacted to it (i.e., reported statements). However, existing work on news summarization almost exclusively focuses on the event details. 
In this work, we propose the novel task of summarizing the reactions of different speakers, as expressed by their reported statements, to a given event. To this end, we create a new multi-document summarization benchmark, \textsc{SumREN}, comprising 745 summaries of reported statements from various public figures obtained from 633 news articles discussing 132 events.\footnote{Data will be available at: \url{https://github.com/amazon-science/SumREN}} We propose an automatic silver-training data generation approach for our task, which helps smaller models like BART achieve GPT-3 level performance on this task. Finally, we introduce a pipeline-based framework for summarizing reported speech, which we empirically show to generate summaries that are more abstractive and factual than baseline query-focused summarization approaches. 


==> camera_ready_sections/benchmark.tex <==


%---------------------------------------------------------------
\label{sec:benchmark}
The SumREN benchmark aims to assist in the development and evaluation of models for the reported speech summarization task. %% [Heba: We mentioned this multiple times before] Each instance in the benchmark contains a set of news articles, a speaker and the reported statements (extracted from the news articles) for that speaker along with the corresponding summary for these statements. 
In this section, we describe the task of reported speech summarization, the benchmark construction process, as well as present statistics of the constructed dataset.


Given a set of news articles about a specific event and the speaker name, the goal is to generate a succinct summary for the statements made by the speaker in the source content. 

%\heng{it will be good to summarize the research challenges for this new task, identify indirect quotation? summarizing conflicting statements, etc.}
%---------------------------------------------------------------
%\subsection{Task Definition}
%\revanth{I feel this is very little content to have as a separate subsection? I think it's okay to just move this into the preceding paragraph?}
%\heba{Good point. I changed/rearranged it.}
%\ken{Your task definition is the description of dataset annotation process. It should be move to the Benchmark construction section. In AAAI, we need a task definition from a system/model perspective. }


%Given a news event, a list of all reported statements (both direct and indirect quotations) from one speaker and collected from multiple news articles related to the news event are provided and the task is to generate a succinct summary (between 40 to 60 words) of the given statements. We ask annotators to first select the salient spans within these reported statements before summarizing them. A salient span is a sub-span within the reported statement that contains the crux of the information presented in the statement. Identifying these spans first ensures that the summary focuses on only the key information from the given input.
%---------------------------------------------------------------
\subsection{Benchmark Construction}
%To create SumREN dataset, we collected a set of news articles discussing major events and followed a two-stage annotation process to first identify all reported statements along with their speakers then to write the summary of the statements.

\label{sec:benchmark-construction}
The first step in our benchmark construction process involves collecting a news corpus discussing a large set of events. We split the news articles according to the discussed event and from each cluster of news articles, we then extract all reported statements along with the speakers of each of these statements. Finally, a summary is written for each group of statements by the same speaker.% about each event. 
%---------------------------------------------------------------
\subsubsection{News Corpus Acquisition:} 
We first identified a list of 132 major news events between 2013-2021 that were mentioned in Wikipedia and other sources.
%\footnote{We use websites such as these: \href{https://en.wikipedia.org/wiki/2021}{link1}, \href{https://www.history.com/topics/21st-century/2020-events}{link2}, \href{https://www.insider.com/news-stories-that-gripped-in-the-world-in-2019}{link3}} 
%\heba{Removed the mention of Google News, please don't add back.}
We then collected a list of news articles discussing these events and retained articles that are present in Common Crawl (CC) News.\footnote{For articles between 2013 and 2016, we relied on WayBack Machine since CC News is not available for these years.} We ended up with a total of 633 news articles corresponding to 132 major events.
%---------------------------------------------------------------

\subsubsection{Reported Statements Annotation:} 
To annotate the reported statements and the speakers, we used Amazon Mechanical Turk and collected three annotations per HIT. The annotation tasks were restricted to annotators in English-speaking countries and who passed the custom qualification test for the corresponding task  -- reported statement span selection or speaker identification.\footnote{Please refer to the appendix for detailed annotation guidelines.}
%\heba{Revanth: Please mention roughly how many workers took the qualification test and how many workers were qualified} 
%Overall, 193 annotators took the qualification test and 23 were qualified. In addition, we blocked spammers that spent less than a specified number of seconds per task or that consistently provided low-quality annotations. 
Overall, 12\% of the annotators that took the test were qualified. In addition, we blocked spammers that spent less than a specified number of seconds per task or that consistently provided low-quality annotations. 
For the reported statement span selection task, annotators were provided with a snippet from the news article and were asked to highlight the spans containing reported statements. Contiguous sentences with statements from the same speaker were considered to be parts of the same reported statement. After collecting the annotations, we grouped reported statements (and associated articles) by a specific speaker about each event.

%\heba{Revanth: We cannot use Cohen's Kappa with MTurk. We have to have only two (and the same) annotators}
%For the reported statement identification and speaker extraction tasks, the inter-annotator agreement had a Cohen's kappa of \textbf{TODO:} X and \textbf{TODO:} Y respectively. 


%---------------------------------------------------------------
\subsubsection{Summary Generation:}
 
For summary generation, we relied on expert annotators since it is a more challenging task and hence less suitable for MTurk. 
Two reference summaries produced by two different annotators were created for each cluster of reported statements. 
An abridged version of the annotation guidelines is presented below and a walk-through example of the annotation process is shown in Figure \ref{fig:summ_example}.
\begin{itemize}[noitemsep]
    \item \textbf{Step 1:} For each one of the given statements, identify the salient spans.
    \item \textbf{Step 2:} Group similar salient spans -- that discuss related aspects of the event -- together and combine these similar spans into a single sentence; \textit{using paraphrasing if needed}.
    \item \textbf{Step 3:} Combine these sentences into a summary.
\end{itemize}
%-----------------------------------------------------------
\subsection{Statistics}
Our benchmark has 745 examples in total, with a train/dev/test split of 235/104/406 respectively. On average, the summaries have a length of 57 words and each summary comes from 5.3 reported statements. 57\% of the examples have a single source news article, with 26\% having 2 source articles and remaining 17\% having 3-5 source articles. The average combined source length is 2,065 words. Overall, the news corpus contains 633 articles with a total of 10,762 reported statements from 3,725 unique speakers. Further, we observe that the summaries in our benchmark are relatively more abstractive compared to existing summarization datasets. Table \ref{tab:dataset_novel_ngrams} shows the percentage of novel n-grams, with \textsc{SumREN} containing considerably higher novel tri-grams and 4-grams. To account for this relatively higher abstractiveness and also variance in generation, each example in our benchmark has two reference summaries.
%\heba{Do we evaluate on one reference summary or on both and report the average performance? I am hoping the latter. We need to clarify this in the write-up}
\begin{table}[!htb]
\footnotesize
    \centering
    \def\arraystretch{1.2}
    \begin{tabular}{l|cccc}
    \hline
    \textbf{Datasets} & \textbf{unigram} & \textbf{bigram} & \textbf{trigram}  & \textbf{4-gram}\\
    \hline
    CNN-DM (S) & 17.0 & 53.9 & 72.0 & 80.3 \\
    NY Times (S) & 22.6 & 55.6 & 71.9 & 80.2 \\
    MultiNews (M) & 17.8 & 57.1 & 75.7 & 82.3 \\
    WikiSum (M) & 18.2 & 51.9 & 69.8 & 78.2 \\
    \hline
    SumREN (M) & 16.8 & 63.1 & 86.4 & 93.4 \\
    \hline
    \end{tabular}
    \caption{Percentage of novel $n$-grams in the reference summaries of different summarization datasets. (S) and (M) denote single and multi-document summarization respectively. Numbers for SumREN are computed by averaging over the two reference summaries. %\heba{How are we calculating these percentages? I assume first averaging (or choosing max) over all reference summaries for a given example then averaging over all examples? I think we need to clarify}
    }
    \label{tab:dataset_novel_ngrams}
\end{table}

%\textbf{TODO: Add Statistics}
%\ken{Need to report the average input length and the summary length. Need to mention we have two references for each sample. Need to describe the abstractiveness stat. in Table 2. }
%---------------------------------------------------------------

\subsection{Silver Training Data Generation}
\label{sec:silver-standard}
%\ken{This should be a part of our methods, better have a section for our methods. }
Given the cost associated with annotating statements and writing summaries, we automatically generate large-scale silver-standard training data for our task. 
%Recent progress \cite{brown2020language, chowdhery2022palm} on large-scale pretrained models have shown impressive performance on downstream NLP tasks in zero-shot settings. Prior work \cite{schick2021generating, liu2022wanli} has leveraged such large-scale models to automatically generate datasets, but mainly for discriminative tasks such as semantic textual similarity and NLI. In this work, 
Specifically, we leverage GPT-3 \cite{brown2020language} to automatically generate abstractive silver-standard summaries of the reported statements. This can be achieved by prompting \cite{liu2021pre}, which involves decomposing the task into an instruction (or a  `prompt') that is then provided to the model along with the input as the context. In our scenario, the input would be the reported statements and a speaker--automatically identified through the reported speech system that we build and describe in Section \ref{sec:reported_extraction} and the prompt would be \textit{``Summarize what $<$speaker$>$ said:''}. Similar to the gold-standard dataset, statements corresponding to the same speaker are grouped together before prompting GPT-3 to generate the summary. Overall, we generate 10,457 examples for our silver training set. 

%---------------------------------------------------------------

%\begin{table*}[!htb]
%\small
%    \centering
%    \begin{tabular}{l|cccc}
%    \hline
%    \multicolumn{1}{l|}{\multirow{2}{*}{Datasets}} & \multicolumn{4}{c}{\% of novel $n$-grams} \\
%    & unigrams & bigrams & trigrams & 4-grams \\
 %   \hline
 %   CNN-DailyMail & 17.0 & 53.9 & 72.0 & 80.3 \\
 %   NY Times & 22.6 & 55.6 & 71.9 & 80.2 \\
%    MultiNews & 17.8 & 57.1 & 75.7 & 82.3 \\
 %   WikiSum & 18.2 & 51.9 & 69.8 & 78.2 \\
 %   \hline
%    SumREN (Human) & & & & \\
 %   \end{tabular}
 %   \caption{Caption}
 %   \label{tab:my_label}
%\end{table*}


%---------------------------------------------------------------
%The task is as follows: Given a list of reported statements relevant to the event, generate a short summary of the reported statements. Since different speakers can talk about different aspects of the event, we limit to summarizing statements from the same speaker, with an aim to ensure coherence in the summary. 
%Here, we list the guidelines for annotating the gold-standard summaries for the reported statements from a speaker. 
%A crucial aspect of creating these summaries is first identifying the salient spans within these reported statements, which we define next.

%\heng{In the paper I'm not seeing anything related to your method on grouping statements, identify salient information, generate final summaries, etc., are you adding those?}





==> camera_ready_sections/conclusion.tex <==
In this work, we introduce a new challenging task of summarizing reported speech in news and release \textsc{SumREN} to promote more research in this direction. %Given competitive performance of end-to-end query-focused summarization approaches, we believe that this dataset can also be used for benchmarking future query-focused systems.
%\heba{Also, I am not sure the sentence ``Given competitive ...'' is clear. You mean even if we do not use the pipeline approach, it can still be used with QFS?} \revanth{The sentence means that, since QFS approaches show good/competitive performance, SumREN can be used to also benchmark future QFS approaches, i.e. used as one of the evaluation datasets in the future for newer/better versions of QFS approaches.}
%\heba{Not sure this statement is needed.}
We propose a pipeline-based framework for summarizing reported statements and show that the proposed approach can generate summaries that are both more factual and abstractive than QFS. 
%
Future work involves improving reported speech extraction performance by leveraging entity-linking and by incorporating character-level features for speaker co-reference resolution. Another direction is to improve the coverage of salient spans in reported statements by adding more explicit control into the generation process. 

%Some of the remaining challenges that we plan on tackling are improving the performance of the reported speech extraction and co-reference resolution systems through utilizing entity-linking as well as incorporating character-level features to identify spelling variations . In addition, we plan on exploring controlled-generation where by conditioning the generated summary on a set of previously clustered salient spans.

==> camera_ready_sections/experiments.tex <==
\label{sec:experiments}

\subsection{Training Setup and Metrics}
\label{sec:train_setup}
 %For training a model on existing news datasets, we use a language model that has been pre-trained for summarization. Specifically, we consider Pegasus \cite{zhang2020pegasus}, which uses a transformer-based \cite{vaswani2017attention} encoder-decoder architecture that has been pre-trained with a self-supervised objective, called \textit{gap-sentence generation}.
%We train Pegasus on each of the three summarization datasets (described in Section \ref{sec:datasets}) and call these models \textit{Pegasus-CNN/DailyMail}, \textit{Pegasus-NewsRoom} and \textit{Pegasus-MultiNews} respectively. We use GPT-3 via the OpenAI Playground\footnote{\href{https://beta.openai.com/playground}{https://beta.openai.com/playground}}. 
We explore two methods for fine-tuning our base summary generation models: Silver Training and Gold Fine-tuning. 
During silver training, the models are fine-tuned on the silver-standard training data. For gold fine-tuning, we add a second fine-tuning step using the gold data. 

For evaluation, we use ROUGE \cite{lin2004rouge} % a commonly used n-gram-based metric for summarization tasks 
and choose the best models based on ROUGE-L performance on the development set.\footnote{We use the \textsc{score\_multi} function from the \textsc{rouge\_score} python package: \url{https://pypi.org/project/rouge-score/}}
%We report ROUGE-1, ROUGE-2 and ROUGE-L scores in our experiments. 
We also report BertScore \cite{bert-score} which leverages pre-trained contextual embeddings from BERT and matches words in candidate and reference sentences by cosine similarity. 
As opposed to ROUGE which measures the lexical similarity between the source and generated summaries, BertScore is capable of capturing the semantic similarity. 
%\heba{For BertScore, do we use the average or maximum of the two reference summaries? We need to clarify in the writeup.}
%\revanth{Bert Score natively supports multiple reference summaries and takes the maximum score. Since we directly use the official implementation, maybe we don't need to mention this explicitly?} \heba{sounds good.} %BertScore has also been shown to correlate with human judgment on sentence- and system-level evaluations. 
%-------------------------------------------------------------------
\subsection{Results} 
Table \ref{tab:model_results} compares the performance of our proposed pipeline-based approach against the QFS baselines with and without fine-tuning using our silver and gold data.
For the baselines, GPT-3 performs best, justifying the choice of using it for generating silver-standard training data. We find that using silver training data for fine-tuning improves the performance of both the query-focused SegEnc and pipeline-based BART considerably, even outperforming GPT-3 in terms of ROUGE. Finally, we see that the models further benefit by fine-tuning on the gold human-annotated training data. 
%\heba{Why don't we have Pipeline (Oracle) for the ``BART'' ``Zero-shot'' and  ``Silver Training data'' only setups?}
%\revanth{Pipeline (Oracle) is only shown for the best/final version of the model. We show it for GPT-3 since we don't finetune GPT-3. For BART, we show it for the best version, which is after gold fine-tuning.}
%\heba{makes sense. I clarified in the write-up}.

We also find that using the pipeline approach, where we first extract the reported statements before passing them to GPT-3, achieves considerably better scores than passing the raw articles to GPT-3. However, GPT-3 has relatively lower ROUGE scores than the smaller models (SegEnc and BART) after gold-fine-tuning. We hypothesize that this could be attributed to the fact that GPT-3 generates more abstractive summaries (as will be shown in Table \ref{tab:generated_ngrams}) thereby leading to higher scores for metrics that are capable of capturing semantic similarity.
%\textbf{TODO: Look at a few conflicting BertScore vs ROUGE examples to explain this. Potentially because GPT-3 is more abstractive hence it might be doing better on semantic scoring.}

In zero-shot settings, the pipeline-based model considerably outperforms query-focused baselines, showing the benefit from explicitly extracting reported statements. However, in both silver training and gold fine-tuning settings, the SegEnc model consistently outperforms the pipeline-based models, suggesting that it may be possible to implicitly identify reported statements within an end-to-end approach. Nevertheless, when using the oracle reported statements, BART surpasses SegEnc -- implying that employing better reported speech and co-reference resolution systems will considerably improve the pipeline-based approach.

%\ken{We should provide some take home message here. For example, in the zero-shot setting, pipeline model outperform query-focused models because the extractor can provide additional knowledge about the statements made by a person and let the generative model to focus on those statements.In the silver and gold training data settings, the SegEnc model consistently outperform the pipeline-based models (without oracles). If we are given the oracle statements, the performance surprass SegEnc, so we suspect that the extractor may propagate error to the abstractor. End-to-end models are more suitable when training data is available. And that's why we analyze the performance of speech extractor in the next section. }
%----------------------------------------------------------------------
\subsubsection{Reported Speech Extraction Performance\\}
Next, we analyze the performance of the proposed reported speech extraction component to identify areas of improvement. %We now evaluate our reported speech extraction component (see Section \ref{sec:reported_extraction}), which forms the first-step of the pipeline-based summarization approach. 
%The evaluation metric is based on character-level offset F1 of the extracted reported speech spans. 
We compare our span tagging approach with a Semantic Role Labeling (SRL) baseline to identify reported statements and the corresponding speakers and evaluate using character-level offset \fscore{} of the extracted span. SRL outputs the verb predicate-argument structure of a sentence such as who did what to whom. Given a paragraph as an input, we filter out verb predicates matching a pre-defined set of cues that signal attribution (e.g., \emph{say}, \emph{believe}, \emph{deny}) and identify these sentences as containing reported statements.\footnote{Full list of used cues is in the appendix of arxiv version.} The sentences encompassing ARG-1 of the predicate are considered as the reported statement and the span corresponding to ARG-0 (agent) is used as the speaker.

\begin{table}[!htb]
\footnotesize
    \centering
    \def\arraystretch{1.2}
    \begin{tabular}{c|ccc|ccc}
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{3}{c|}{\textbf{Dev}} & \multicolumn{3}{c}{\textbf{Test}} \\
    %\cline{2-7}
    & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
    \hline
    SRL& 84.3 & 42.7 & 56.7 & 83.3 & 40.8 & 54.8\\
    + co-reference & 82.2 & 68.1 & 74.5 & 83.1 & 68.3 & 75.0\\
    \hline
    Span Tagging & 80.3 & 48.6 & 60.5 & 80.2 & 45.0 & 57.6\\
    + co-reference & 78.7 & 69.9 & 74.1 & 78.2 & 73.0 & 75.5\\
    
    
    \hline 
    \end{tabular}
    \caption{Performance (in \%) of different approaches for identifying reported statements corresponding to a given speaker for the summaries in SumREN. ``\textit{+ co-reference}'' corresponds to adding co-reference resolution for the speaker mention extracted by the system.}
    \label{tab:summary_statements}
\end{table}

As shown in Table \ref{tab:summary_statements}, our proposed span tagging model outperforms SRL, especially in terms of recall which ensures better coverage of information for the summarization step. We also find that incorporating co-reference resolution for speaker identification considerably improves recall with almost the same or slightly lower precision.
Table \ref{tab:all_statements} measures the performance of the proposed span-tagging approach for speaker extraction against the SRL baseline. We report both string exact-match and \fscore{}, both of which are commonly used in extractive question answering \cite{rajpurkar2016squad}.
We find that the performance of different approaches for identifying the speaker of a given reported statement improves significantly when using co-reference resolution. This is crucial for correctly grouping statements from the same speaker together. 
%----------------------------------------------------------------------

\begin{table}[!htb]
\footnotesize
    \def\arraystretch{1.2}

    \centering
    \begin{tabular}{c|cc|cc}
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c|}{\textbf{Dev}} & \multicolumn{2}{c}{\textbf{Test}} \\
    %\cline{2-6}
    & \textbf{Exact-Match} & \textbf{F1} & \textbf{Exact-Match} & \textbf{F1} \\
    \hline 
    SRL & 20.8 & 48.1 & 16.1 & 44.4\\
    + co-reference & 62.9 & 73.7 & 69.1 & 77.1 \\
    \hline
    Span Tagging & 22.3 & 51.2 & 18.8 & 49.3 \\
    + co-reference & 63.3 & 74.8 & 69.8 & 78.4 \\
    \hline
    
    \end{tabular}
    \caption{Performance (in \%) of the proposed span tagging component -- against the baseline -- on identifying the speakers corresponding to the given reported statements with and without co-reference resolution. %\heba{Please explain the difference between Exact-Match and F1.}
    }
    \label{tab:all_statements}
\vspace{-0.75em}
\end{table}
%To further quantify the benefit of using co-reference resolution for the speaker mention, we also measure the speaker extraction performance--evaluated based on string exact-match and \fscore{}, both of which are commonly used in extractive question answering \cite{rajpurkar2016squad}--and present the results in Table \ref{tab:all_statements}.
%
%----------------------------------------------------------------------
%----------------------------------------------------------------------
\subsubsection{Parameter-Efficient versus Direct Fine-tuning\\} 
%\revanth{Should we move this subsubsection to the appendix to save space? We can add a line in the main paper saying: ``We also experimented with parameter-efficient fine-tuning approaches on our benchmark. Please refer to the appendix for more details.}
%\ken{The motivation of this section is not very clear. Should say sometime like since we investigate extractor performance in the previous section. In this section, we explore and evaluate the performance of different design choices in the abstractor model.}
%In this section, we experiment with different choices for fine-tuning the summarization model in our pipeline-based approach.
%\heba{Revanth, please make sure to add X--\% of trainable parameters below.}
In addition to full fine-tuning methods, we also explore leveraging parameter-efficient fine-tuning approaches to directly fine-tune on the small-scale gold training data. We use LORA \cite{hu2021lora}, an efficient fine-tuning technique that injects trainable low-rank decomposition matrices into the layers of a pre-trained model. Table \ref{tab:pe_approaches} compares the performance of three different fine-tuning strategies, namely \emph{Full FT} (silver training + gold fine-tuning), \emph{Gold FT} (direct gold fine-tuning) and PE FT (parameter-efficient gold fine-tuning). 
We find that the benefit of incorporating the silver-standard training data can be seen from the fact that Full FT considerably outperforms Gold FT. We also observe that \emph{PE FT} with LORA, which fine-tunes only 0.3\% of model parameters, can achieve a comparable performance to Full FT while also consistently outperforming \emph{Gold FT}. 
This shows that parameter-efficient fine-tuning is effective for our pipeline-based reported speech summarization framework, with future work potentially benefiting from better PE approaches \cite{liu2021p}. 
%\ken{Should give take home message, e.g., parameter-efficient method is effective in our task?}
%----------------------------------------------------------------------
\begin{table}[!htb]
\footnotesize
    \def\arraystretch{1.2}
    \centering
    \begin{tabular}{l|cc|cc}
    \hline
    \multicolumn{1}{c|}{} &  \multicolumn{2}{c|}{\textbf{Dev}} &  \multicolumn{2}{c}{\textbf{Test}} \\
    & \textbf{R-1/2/L} & \textbf{BertS} & \textbf{R-1/2/L} & \textbf{BertS}  \\
    \hline
    Full FT & 51.1/24.2/35.9 & 42.3 & 47.8/20.2/32.3 & 39.6\\
    \hline
    Gold FT & 50.0/23.9/35.1 & 40.9 & 47.2/19.5/31.4 & 38.4\\
    \hline
    PE FT & 50.7/24.6/36.1 & 42.0 & 47.8/20.2/31.8 & 39.4\\
    \hline
    \end{tabular}
    \caption{Comparison of performance of parameter-efficient fine-tuning for BART when used for summarization with oracle reported statements. \textit{Full FT} corresponds to silver training + gold FT.}
    \label{tab:pe_approaches}
\end{table}

\begin{table*}[]
\scriptsize
\def\arraystretch{1.4}
    \centering
    % \begin{tabular}{p{54em}}
    \begin{tabular}{p{69em}}
    \multicolumn{1}{c}{\textbf{Event}: 2017 Solar Eclipse \hspace{1.5em} \textbf{Speaker}: Jamie Yuccas \hspace{1.5em} \textbf{News Article}: \url{https://www.cbsnews.com/news/solar-eclipse-august-21-2017-across-america}}\\
    \hline
    % \hspace{20em}\textbf{Reported Statements}\\
    \hspace{30em}\textbf{Gold Reported Statements}\\
    \hline
    ``They're expecting about a million people to enter the state, a million out-of-towners are supposed to come to the state of Oregon,'' said CBS News correspondent Jamie Yuccas. ``Where we're located in Madras, they're expecting between 100,000 and 200,000 people.''\\
    \hdashline
    She said the local residents have been ``really, really nice and accommodating.''\\
    \hdashline
    ``What the mayor said to me was kind of funny,'' Yuccas said. ``He said 'you know, I think it's going to be one of those situations that you might not get your newspaper, you might not have your daily Starbucks and if that happens, I guess it's a first-world problem, and you're going to have to figure out your own survival skills.'''\\
    \hdashline
    She laughed, saying ``there are going to be some minor inconveniences, but I actually think they had a pretty good plan together.''\\
    %\hline
    \hline
    \textbf{SegEnc (QFS):} Jamie Yuccas has said that the local residents of Madras, Oregon have been very accommodating towards people who are coming to see the solar eclipse. She laughed when she heard that the mayor of the town thought it would be a first-world problem if the eclipse did not occur. She said that they are expecting about a million people to enter the state, and that a million out-of-towners are supposed to come to the state. \\
    \hline
    \textbf{GPT-3 (QFS):} Jamie Yuccas is a CBS News correspondent who is reporting from Madras, on the upcoming solar eclipse. She says that the city is expecting between 100,000 and 200,000 visitors for the event, and that the locals have been very accommodating. Yuccas also says that the eclipse is expected to be the most observed eclipse in history.\\
    \hline
    \textbf{GPT-3 (Pipeline):} Jamie Yuccas said that the city of Portland is expecting about a million out-of-towners to come to Oregon for the eclipse, and that the locals have been very accommodating. She said that the mayor told her that there may be some minor inconveniences, but that they have a good plan in place.\\
    \hline
    \textbf{BART (Pipeline):} According to the correspondent, the state of Oregon is expecting a million people from out-of-towns to come to the state, and the local residents have been very nice and accommodating. However, there will be some minor inconveniences, but the state had a good plan in place.\\
    \hline
    \textbf{Gold:} Jamie Yuccas said that a million tourists are supposed to come to the state of Oregon and between 100,000 and 200,000 people are expected in Madras, where she is located. She also mentioned minor inconveniences could occur derived from the event, but overall, they had a good plan set in place.\\
    %\hdashline
    %\textbf{Gold 2:} Jamie Yuccas said the people from Madras were very warm and welcoming while preparing themselves for the 100,00 to 200,000 visitors they are expecting to attend the event this 2017. Jamie Yuccas also said a few little drawbacks were expected.\\
    \hline
    \end{tabular}
    \caption{Model outputs for an example in SumREN, along with the gold reported statements. Summaries from the QFS approaches contain factually inconsistent fragments, while those from  pipeline-based
approaches better match the gold summary.}
    \label{tab:analysis}
    \vspace{-0.95em}
\end{table*}


%----------------------------------------------------------------------
\subsubsection{Abstractiveness and Factuality of Generated Summaries \\}
We investigate the effect of using silver and gold data for fine-tuning, on both the abstractiveness and factuality of generated summaries. There is generally a trade-off  between abstractiveness and factual consistency of the summary against the source input~\cite{dreyer2021analyzing}. Hence, the goal of any abstractive summarization system is to generate more abstractive summaries while maintaining a high level of factual consistency with the source.
\begin{table}[!htb]
\footnotesize
\def\arraystretch{1.2}
    \centering
    \begin{tabular}{c|c|c|cccc}
    \hline
     & \textbf{Model} & \textbf{Setting} & \textbf{Uni} & \textbf{Bi} & \textbf{Tri} & \textbf{MINT}\\
    \hline
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{QFS}}} & \multicolumn{1}{c|}{\multirow{3}{*}{SegEnc}} & Zero-Shot & 1.0 & 6.6 & 13.1 & 11.1\\
    %\cline{3-6}
   & & + Silver Train & 2.8 & 22.8 & 39.3 & 31.2\\
   %\cline{3-6}
    & & + Gold FT & 3.6 & 26.6 & 46.6 & 38.4\\
    \cline{2-7}
    & GPT-3 & Zero-Shot & 3.8 & 26.2 & 44.2 & 38.9\\
    \hline
    %\hline
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Pipeline}}} & \multicolumn{1}{c|}{\multirow{3}{*}{BART}} & Zero-Shot & 1.9 & 11.5 & 20.5 & 15.3\\
    %\cline{3-6}
   & & + Silver Train & 3.3 & 24.8 & 41.6 & 32.9\\
   %\cline{3-6}
    & & + Gold FT & 4.7 & 30.6 & 52.1 & 43.5\\
    \cline{2-7}
    & GPT-3 & Zero-Shot & 5.7 & 35.2 & 56.6 & 49.6\\
    \hline
    \end{tabular}
    \caption{Abstractiveness and novelty scores -- measured by \% of novel ngrams -- of the generated summaries using silver and gold data for fine-tuning the models. The novelty is computed with respect to the source news articles.}
    \label{tab:generated_ngrams}
    \vspace{-0.3em}
\end{table}


%----------------------------------------------------------------------
For abstractiveness, we measure it through the percentage of novel $n$-grams (uni, bi and tri-grams), as well as MINT (\emph{M}etric for lexical \emph{IN}dependence of generated \emph{T}ext) \cite{dreyer2021analyzing} which is computed based on the n-gram precision and longest common sub-sequence length of the generated summary. 
As shown in Table \ref{tab:generated_ngrams}, we find that models in zero-shot settings are considerably more extractive, and that abstractiveness of generated summary significantly increases from both silver training and gold fine-tuning. % potentially due to the summaries in the gold and silver train data (generated from GPT-3) being relatively more abstractive. 
Further, we notice that our pipeline-based approach is considerably more abstractive than the QFS approach, demonstrating that incorporating an explicit statement extraction component helps the summarization model focus on paraphrasing and synthesizing the selected statements into the summary.
%\ken{Need to explain it, e.g., in pipeline-based approach, extractor handles most of the content selection, generative model can focus on paraphrase and synthesize the selected statements into summary. }
%----------------------------------------------------------------------


\begin{table}[!htb]
\footnotesize
\def\arraystretch{1.2}
    \centering
    \begin{tabular}{c|c|ccc}
    \hline
    \textbf{Approach} & \textbf{Model} & \textbf{FactCC} & \textbf{Entity P} & \textbf{MINT}\\
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{QFS}} & GPT-3 & 45.4  & 61.7 & 38.9 \\
    
   & SegEnc  & 50.8  &  \textbf{75.4} & 38.4\\
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{Pipeline}} & GPT-3 & 50.2 & 73.2 & \textbf{49.6}\\

   & BART  & \textbf{52.1} & 74.6 & 43.5\\
    \hline
    %\hline
    \multicolumn{1}{c|}{\multirow{2}{*}{\demph{Pipeline (Oracle)}}} & \demph{GPT-3} & \demph{52.0}  & \demph{78.9} & \demph{51.3}  \\
 
   & \demph{BART} & \demph{55.0} & \demph{84.6} & \demph{44.0}  \\
    \hline
    \end{tabular}
    \caption{Comparison of factuality (measured by FactCC and Entity Precision) of generated summaries relative to abstractiveness (measured by MINT). Models considered are after silver train + gold FT, except GPT-3 which is not fine-tuned.}
    \label{tab:factuality}
    \vspace{-0.3em}
\end{table}

\begin{comment}
\begin{table*}[]
\scriptsize
\def\arraystretch{1.4}
    \centering
    % \begin{tabular}{p{54em}}
    \begin{tabular}{p{69em}}
    \multicolumn{1}{c}{\textbf{Event}: Disappearance of journalist Jamal Khashoggi \hspace{4.5em} \textbf{Speaker}:  Robert Mahoney} \\
    \hline
    % \hspace{20em}\textbf{Reported Statements}\\
    \hspace{30em}\textbf{Gold Reported Statements}\\
    \hline
    \textbf{Statement 1:} ``The worrying trend that we see is a crackdown on critical and independent journalism in Saudi and about Saudi,'' Robert Mahoney, Deputy Executive Director of CPJ, told CBS News. ``It is a very repressive place.''\\
    \hdashline
    \textbf{Statement 2:} He said that there is no surprise that Riyad is looking to quash criticism, but this case is beyond the sad but true usual jailing of journalists.\\
    \hdashline
    \textbf{Statement 3:} ``This is an incredible escalation if these stories are true,'' Mahoney said. ``We have had cases where journalists are killed in another country, but no one as prominent as this, not a U.S. resident who was writing for the Washington Post. He is a journalist but he was also from the Saudi establishment before the present Crown Prince came.''\\
    \hdashline
    \textbf{Statement 4:} Mahoney said that the disappearance of Khashoggi is ``designed in a very brutal way to send a message `if you speak out against the Saudi government, if it could happen to him, it could happen to you.'''\\
    \hdashline
    \textbf{Statement 5:} ``With no body, there is no crime ... is the way the Saudis are treating the case right now'', Mahoney said. \\
    \hdashline
    \textbf{Statement 6:} The Committee to Protect Journalists Deputy Executive Director Robert Mahoney said in a statement that the group was ``alarmed'' by the reports that Khashoggi may have been killed inside the consulate.\\
    \hdashline
    \textbf{Statement 7:} ``The Saudi authorities must immediately give a full and credible accounting of what happened to Khashoggi inside its diplomatic mission,'' Mahoney said. ``The country has stepped up its repression of critical journalists in the past year at home. We hope this has not now spread abroad.''\\
    \hline
    \textbf{BART (Pipeline):} Robert Mahoney, Deputy Executive Director of CPJ, said that the disappearance of journalist Jamal Khashoggi was a result of a crackdown on critical and independent journalism in Saudi Arabia, and that if the reports of his disappearance are true, it would be an escalation beyond the usual jailing of journalists. Mahoney expressed concern that the Saudi authorities must give a full and credible account of what happened to the journalist inside the consulate. \\
    \hline
    \textbf{Human:} Robert Mahoney said the reports of Jamal Khashoggi's disappearance alarmed the group, standing as the most prominent case of the sad but real jailing and killing of journalist in an attempt to crack down critical and independent journalism in and about Saudi designed brutally as a message to other journalists. Mahoney demands a full account from Saudi authorities of Khashoggi's whereabouts despite their evasive approach towards the case claiming the absence of a body.\\
    %\hdashline
    %\textbf{Gold 2:} Jamie Yuccas said the people from Madras were very warm and welcoming while preparing themselves for the 100,00 to 200,000 visitors they are expecting to attend the event this 2017. Jamie Yuccas also said a few little drawbacks were expected.\\
    \hline
    \end{tabular}
    \caption{Example output from the proposed BART-based pipeline, along with the gold reported statements and corresponding reference summary. The human summary has considerably higher coverage of the input statements than the BART summary.}
    \label{tab:coverage_example_1}
\end{table*}
\end{comment}

For factuality, we use FactCC \cite{kryscinski2020evaluating}, which \citet{pagnoni2021understanding} show to correlate most with human factuality labels. In addition, Entity Precision~\cite{DBLP:conf/eacl/NanNWSZZMX21} is calculated based on the percentage of named entities in the generated summary that are present in the gold reported statements.
In Table \ref{tab:factuality}, we observe that while our proposed pipeline-based approach is considerably more abstractive than the QFS baselines, it still maintains high entity precision and a slightly higher FactCC score. As expected, we see that using gold (oracle) statements as input to the summarization step improves the factual consistency scores.
%----------------------------------------------------------------------
%----------------------------------------------------------------------
%Further, we observe that GPT-3 is more abstractive in the pipeline setting, meaning it tends to be more extractive when presented with the entire news articles (in the query-focused setting), whereas it paraphrases more when presented with lesser content (just the extracted reported statements).
%----------------------------------------------------------------------

%===================================================================
\subsubsection{Human Evaluation\\}

We also performed a human study of the summaries generated using GPT-3 via both pipeline-based and QFS approaches. We chose GPT-3 summaries since they have consistently high scores across Rouge-L, BertScore and abstractiveness. The summaries were evaluated on a scale of 1-3 for factual consistency, informativeness and coherence\footnote{Detailed guidelines are in the appendix of the arxiv version.}. Evaluation for \textit{factual consistency} involves looking for major or minor factual errors in the summary, \textit{informativeness} is about how well the summary expresses the main point of the reported statements, and \textit{coherence} is mainly checking whether the summary has a good flow and facts are presented in a logical order. The annotations were crowd-sourced via MTurk. Table \ref{tab:human_study} shows results from the human study. We find that summaries from the pipeline-based approach have considerably better factual consistency with the ground-truth reported statements, with slight improvements in informativeness. Concurring with recent observations \cite{goyal2022news, zhang2023benchmarking} on the quality of summaries from large language models, we see that the summaries based on the two approaches, which both come from GPT-3, are very coherent.

\begin{table}[!htb]
\footnotesize
\def\arraystretch{1.2}
    \centering
    \begin{tabular}{c|ccc}
    \hline
    \textbf{Approach} & \textbf{Consistent} & \textbf{Informative} & \textbf{Coherent}\\
    \hline    
    GPT-3 (QFS) & 2.76 & 2.92 & 2.99\\
    GPT-3 (Pipeline) & 2.92 & 2.95 & 2.99\\    
    \hline
    \end{tabular}
    \caption{Results from human study on summaries from GPT-3 via pipeline-based and QFS approaches, when evaluated for factual consistency, informativeness and coherence.}
    \label{tab:human_study}
    \vspace{-0.3em}
\end{table}

\subsection{Manual Error Analysis}

Table \ref{tab:analysis} shows outputs from different models for an example in \textsc{SumREN}. We see that summaries from the query-focused approaches contain factually inconsistent fragments: SegEnc output suggests that the mayor \textit{``thought it would be a first-world problem if the eclipse did not occur''} whereas the mayor actually refers to \textit{``people not getting their newspapers or their daily Starbucks''} as the first-world problems; GPT-3 (QFS) misattributes the statement \textit{``the eclipse is expected to be the most observed eclipse in history''}. On the other hand, summaries from pipeline-based approaches match the gold summary better, with those from BART and GPT-3 (Pipeline) being fairly similar in quality.

%We manually examined outputs from different models and found that the summaries from the query-focused approaches contain factually inconsistent fragments. For example, a summary from SegEnc  says that a given speaker \textit{``thought it would be a first-world problem if the eclipse did not occur''}, whereas the first-world problem the speaker mentioned in the source text is people not getting their newspapers or their daily Starbucks as the first-world problems. On the other hand, GPT-3 frequently suffers from  mis-attribution in the generated summary. Finally, and confirming the quantitative results in Tables \ref{tab:generated_ngrams}, we find SegEnc to be highly extractive with some sentences in the generated summary having considerable overlap with the input statements. On the other hand, we see that summaries from pipeline-based approaches match the gold summary better, with those from BART and GPT-3 (pipeline) being fairly similar in quality.\footnote{Examples of model outputs are provided in the Appendix.}

%\heba{NIT: Please make sure that we stick to the same tense (either past or present) when describing what we did (e.g., found, analyzed). I changed in some places, but I might have missed some. Also, footnotes should come after punctuation.}

We also analyzed some of the errors made by the reported speech extraction component of the proposed pipeline. As Table \ref{tab:model_results} shows, there is still a considerable room for improving our pipeline-based approach with better reported speech extraction systems. We found that the same entity can be referred to by different aliases that the co-reference system sometimes fails to capture (e.g., ``Islamic State'' and ``ISIS'' or ``Anthony M. Kennedy'' and ``Justice Kennedy''). 
%
Utilizing entity-linking \cite{ayoola2022refined} will likely improve co-reference for entities with different aliases. In addition, we found that spelling variations; e.g., Nikos vs. Nicos, Muhammad vs. Mohammed or Sergey vs. Sergei, were also frequently missed by the system. We believe that incorporating character-level features into the co-reference resolution system will make it more robust to such variations.

%\subsubsection{Improving coverage of generated summaries}

Finally, to analyze the informativeness of the generated summaries, we calculated the percentage of input reported statements covered in the output summary. To obtain alignments between source-summary pairs, we leveraged SuperPAL \cite{ernst2021summary} which aligns OpenIE-extracted \cite{stanovsky2018supervised} propositions in the generated summary with those in the source sentences. We found %\footnote{We provide qualitative examples in the appendix.} 
that human summaries cover considerably more percentage of the input reported statements (57.5\%) compared to summaries from BART (51.2\%) and GPT-3 (46.5\%) in \textit{Pipeline (Oracle)} settings. 
%Table \ref{tab:coverage_example_1} shows one such qualitative example where the human summary covers information from statements 1, 2, 4, 5, 6 and 7, whereas the BART model output only covers statements 1, 2, 3 and 7. 
In order to explicitly improve coverage, future work can explore incorporating more control into the generation output by clustering the salient spans within the reported statements and separately generating summaries for each cluster, similar to \citet{ernst2022proposition}.


\begin{comment}

\subsection{Human evaluation}
In addition to automatic evaluation, we performed a human evaluation of the generated summaries. 
Annotators were presented with the summaries along with the gold reported statements and asked to rank the summaries based on \textit{informativeness} and \textit{readability}. 
In addition, they were given a binary choice of whether the summary was \textit{factually consistent} with the reported statement. 
We used informativeness to identify whether the summary sufficiently captured the salient information and readability as a combination of commonly used fluency and coherency\footnote{Detailed annotation guidelines are shown in the appendix.}. 

We randomly picked 50 examples from the test set for our evaluation. 
For readability and informativeness, we use the Bojar score~\cite{DBLP:conf/wmt/BojarEPZ11} to aggregate the rankings provided by annotators. Bojar score computes the ratio of samples that a system is ranked better than all other systems and is widely adopted by WMT tasks~\cite{DBLP:conf/iwslt/Koehn12}. 
For factual consistency, we report the ratio of consistent samples. 
Table \ref{tab:human_eval} shows the results of human evaluation of summaries from query-focused and pipeline-based approaches. We observe that ... \textbf{TODO}
\heba{How come the human summaries are worst in terms of informativeness and factual consistency. This doesn't seem right}
%----------------------------------------------------------------------
\begin{table}[!htb]
\footnotesize
    \centering
    \begin{tabular}{c|l|c|c|c}
    \hline
    && Readability & Informativeness & Fact. Consist.\\
    \hline
    \parbox[t]{2.0mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{QFS}}} & SegEnc & 67.8 & 63.8 & 88.0 \\
   & GPT-3 & 59.0 & 26.2 & 82.0 \\
    \hline
   \parbox[t]{2.0mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{P}}} & GPT-3 & 68.2 & 43.4 & 86.0 \\
   &  BART & 42.8 & 55.4 & 80.0 \\
    \hline
   & Human & 81.3 & 56.1 & 76.0 \\
   \hline
    \end{tabular}
    \caption{Human evaluation of model outputs compared against human summaries. (QFS) and (P) correspond to query-focused and pipeline-based approaches respectively.}
    \label{tab:human_eval}
\end{table}

\end{comment}

==> camera_ready_sections/introduction.tex <==
%%Heba: This is redundant so I commented out
%%In modern journalism, reported speech serves as a central resource for tracking public figures' stance, opinions and worldviews, especially on complex events. Further, reported statements\footnote{We use the terms reported statements and reported speech interchangeably in this paper.} can be a means to learn more information about these events from those directly involved or affected by it. Existing news summarization approaches \cite{hermann2015teaching, narayan2018don, fabbri2019multi, martschat2018temporally, li2021timeline} have largely focused on summarizing the details of events in news, and have neglected the responses from the public figures toward these events.

%\heba{Revanth: I commented the first Table out since we already have a detailed walk-though example in Figure 1. Also, I think we should move Table 8 (that has the system outputs) to the appendix and just summarize in the discussion.}
%\revanth{Should we cut-down on text first and have moving Table 8 into the appendix as a last resort? I think we can still cut considerable content in related work and experiments}
%\heba{Sounds good. Will go through the experiments now though I still think Table 8 is too big and should likely be summarized in the text.}

\begin{table}[!htb]
\renewcommand{\arraystretch}{0.9}
% \footnotesize
\scriptsize
    \centering
    % \begin{tabular}{|p{25em}|}
    \begin{tabular}{|p{32em}|}
                 \hline
                %  \multicolumn{1}{|c|}{\textbf{Event: \textit{Power Outage in Texas} \hspace{2em}Speaker: \textit{Nateghi}}} \\
                 \multicolumn{1}{|c|}{\textbf{Event: \textit{Power Outage in Texas} \hspace{4em}Speaker: \textit{Nateghi}}} \\
                 \hline
                 \hline
                 \multicolumn{1}{|c|}{\textbf{Reported Statements}}\\
                 \hline
                 An issue facing all power grid operators, Nateghi of Purdue said, is adequately preparing for changes in climate. \\
                 \hline
                 They're also not taking into account inter-dependencies in the system: You need water to generate electricity, and you need electricity to transport water, and so on and so forth, Nateghi said. \\
                 \hline
                 And when the system is really stressed from an extreme event like it is in Texas, then we're seeing natural gas shortages which exacerbate the whole impact, she said. \\
                 \hline
                 Nateghi, who researches sustainability and resilience of infrastructure, said other solutions such as upgraded equipment and infrastructure may not be as cost-effective, but are still crucial.\\
                 \hline
                 ``If we continue down the paradigm of what we've done before we are going to see more extremes,'' Nateghi said. ``These stories are going to just keep playing, and perhaps even more frequently.'' \\
                 \hline
                 \hline
                 \textbf{Summary:} \textit{Nateghi said that interdependencies in the system are not being considered, and the problem of gas shortages could be seen in the power outage in Texas. Solutions such as upgraded equipment and infrastructure maybe less cost-effective but crucial. She also said that power grid operators needed to make changes before extreme situations became more frequent.}\\
                 \hline
\end{tabular}
    \caption{An example from \textsc{SumREN} showing reported statements from the speaker ``Nateghi'' about the ``Power outage in Texas'' along with the corresponding summary.}
    \label{tab:intro_ex}
    \vspace{-1.0em}
\end{table}
In news, attribution occurs when the journalist reports the statements of a third party either by directly quoting them (i.e., direct quotation) or paraphrasing what they said (i.e. indirect quotation). Reported speech serves as a central resource for tracking public figures' stance, opinions, and worldviews, making it of general interest to news readers. For example, readers are likely to be interested in knowing President Biden's view on the 2022 Ukraine crisis or the latest guidance from the Center for Disease Control and Prevention regarding a new COVID-19 variant. In addition, reported statements cover a significant portion of the information presented in news articles -- as part of our annotation exercise (described later in section \ref{sec:benchmark-construction}), we found that 45\% of the overall article content corresponds to reported statements. 
%As part of our annotation exercise (described later in section \ref{sec:benchmark-construction}), we found that 42\% of the paragraphs in news articles and 45\% of the overall content. %\footnote{These statistics were averaged over 814 news articles with 28,664 paragraphs in total.}
%corresponds to reported statements. 
However, current news summarization datasets such as CNN-DM \cite{hermann2015teaching}, Multi-News \cite{fabbri2019multi}, and Timeline$_{100}$ \cite{li2021timeline} largely disregard summarizing these reported statements. 

%Figure \ref{fig:intro_ex} shows an example news article with information presented about events highlighted in red and the reported statements highlighted in blue. Existing news summarization tasks mainly deal with summarizing the details provided in red, while the content in blue provides information about what popular figures have said regarding these events. These reported statements could be of general interest to a wide audience, for example, news readers would be interested in knowing what President Biden has said regarding the 2022 Ukraine crisis or what the Center for Disease Control and Prevention has said about the new Delta variant. \heng{the colors are not visible in printed version, so you may want to label them instead}



%\begin{figure}[!htb]
%    \centering
%    \includegraphics[width=1.0\linewidth]{figures/statements.png}
%    \caption{Figure showing statements (in red) that describe the events and the reported speech (in blue) for a news article\footnotemark relating to the winter storm in Texas. \heng{the color is indistinguishable in printed versoin. you may want to other formats}}
%    \label{fig:intro_ex}
%\end{figure}

%\footnotetext{\href{https://www.foxnews.com/us/warmer-temperatures-brings-welcome-relief-to-texas-and-other-southern-states-following-deadly-winter-storm}{Original news article}}
\begin{comment}
\begin{table*}[h]
\footnotesize
   \small
    \centering
    \begin{tabular}{p{37em}|c|p{6em}}
      \multicolumn{1}{c|}{\textbf{Statement}} & \textbf{Type} & \multicolumn{1}{c}{\textbf{Speaker}}\\
      \hline
      ``We're stuck here until we can get some reprieve from ERCOT,'' Sargent said. & Direct & Sargent \\
      \hline
      ``One way to gather this water is to collect water dripping for your faucets to prevent freezing,'' the City of Pflugerville said in a tweet. & \multirow{2}{*}{Direct} & City of Pflugerville \\
      \hline
      Sir Alex Ferguson said the proposals would be a move away from '70 years of football history & Indirect & Alex Ferguson \\
      \hline
      Abbott urged residents to shut off water to prevent more busted pipes and preserve municipal system pressure. & \multirow{2}{*}{Indirect} & \multirow{2}{*}{Abott} \\
      \hline
    \end{tabular}
    \caption{Some examples of direct and indirect quotations that occur in news articles along with the speakers.}
    \label{tab:quotations}
\end{table*}
\end{comment}
To bridge this gap, we introduce the new task of \textbf{Sum}marizing \textbf{R}eported speech about \textbf{E}vents in \textbf{N}ews and create a new benchmark, \textsc{\textbf{SumREN}}, for this task. Formally, given a set of news articles related to a specified event, the task is to summarize the statements made by a given speaker about this event (e.g., ``What did Chuck Schumer say about passing the Inflation Reduction Act of 2022?"). The aim of the task is to provide news readers with the reactions of various public figures towards different events. Table \ref{tab:intro_ex} shows an example from \textsc{SumREN}, along with the reported statements and the corresponding reference summary. %\heba{Should we add the two reference summaries instead of one?}


Summarizing reported speech in news brings a set of unique challenges. 
As opposed to traditional news summarization datasets where the most salient information about the event is normally discussed in the first few sentences of a given article, generally referred to as ``\textit{lead bias}'' \cite{jung2019earlier, zhu2021leveraging}, reported speech from the same speaker can be scattered across the entire article. Statements can be split across multiple sentences (i.e., ``running quotations'') and speakers are often referred to by their nominal and pronominal mentions, requiring modelling of long-term dependencies and reliable co-reference resolution.   %An example of such case is shown in Table \ref{tab:intro_ex} where the given speaker is mentioned both with her name  \textit{Nateghi} and as ``\textit{she}''. 
%An example of such case is shown in Table \ref{tab:intro_ex} where the first sentence in the summary requires combining salient points from multiple statements.
Additionally, generating concise summaries from a set of reported statements requires a higher level of abstraction. This is also verified empirically, as we find that summaries in \textsc{SumREN} are considerably more abstractive compared to existing news summarization datasets, as shown in Table \ref{tab:dataset_novel_ngrams}. %\revanth{Added the below statement since we mention factual consistency a lot in the paper}
Finally, factual consistency is paramount in reported speech summarization, as misquoting or misrepresenting statements from public figures can be particularly harmful.

To address the above challenges, we propose a pipeline-based approach for the task of summarizing reported speech in news articles. The pipeline involves first identifying individual statements and corresponding local speaker mentions, then resolving speaker mentions globally using co-reference resolution to group statements from the same speaker together, and finally summarizing the extracted reported statements by the given speaker. 
%To address the above challenges, we propose a pipeline-based approach for the task of summarizing reported speech in news articles which first identifies individual statements and corresponding local speaker mentions, then resolves speaker mentions globally using co-reference resolution to group  statements from the same speaker together, and finally summarizes the extracted reported statements by the given speaker. 
We hypothesize that, in a pipeline-based framework, having an explicit extractive component that can identify relevant context helps the summarization model better attend to the key information from the given articles.
%, leading to more concise summaries. \heba{I think we should report the median and/or average length of generated summaries from each approach, probably in Table \ref{tab:factuality}, to show that the pipeline approach results in more compression.}
%\revanth{Length of generated summaries is a hyperparameter tuned based on Rouge-L for dev set. The maximum number of output words in RelReg, SegEnc, GPT-3, and our pipeline are set to 384, 256, 200, and 90, respectively. How should we best convey this information?}
%\heba{This is the maximum length though not the actual, right? Either way, we should probably remove ``leading to more concise summaries'' since we don't have any numbers to support it.}
 

In addition, we introduce a cost-effective approach to generating training data for the reported speech summarization task. Specifically, we leverage large-scale pre-trained language models, such as GPT-3~\cite{brown2020language}, to generate silver-standard summaries for statements obtained from automatic reported speech extraction systems. This follows recent work that uses large language models to create training data~\cite{schick2021generating}, although previously explored for discriminative tasks such as Natural Language Inference. We show that training with such silver-standard data can help smaller language models, such as BART \cite{lewis2020bart} achieve GPT-3-level performance on this task. \\ \\
To summarize, the contributions of this work include:
\begin{itemize}[noitemsep]
    \item introducing a new challenging task of summarizing reported speech about events in news and releasing the first multi-document summarization benchmark, \textsc{SumREN}, for the task. \textsc{SumREN} contains 745 instances annotated over 633 news articles discussing 132 events, %, with summaries that are considerably more abstractive than existing summarization datasets.
    \item empirically demonstrating that large-scale language models can be leveraged to create cost-efficient silver-standard training data for the reported speech summarization task,
    \item proposing a pipeline-based reported speech summarization framework and showing that it is capable of generating summaries that are considerably more abstractive than query-focused approaches, while also improving the factual consistency of the generated summaries with the source documents.
    
\end{itemize}

==> camera_ready_sections/models.tex <==
\begin{table*}[!htb]
\small
    \centering
    \def\arraystretch{1.2}
    \begin{tabular}{p{4.7em}|c|c|cccc|cccc}
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Setting}}}&\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Approach}}} & \multicolumn{4}{c|}{\textbf{Dev}} &  \multicolumn{4}{c}{\textbf{Test}} \\
    %\cline{4-11}
    & & & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{BertScore} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{BertScore}  \\
    \hline
     \multirow{3}{*}{\parbox{4.7em}{\centering Baselines (Zero-shot)}} & GR-SUM & \multicolumn{1}{c|}{\multirow{4}{*}{QFS}} & 38.73 & 15.32 & 24.70 & 16.45 & 35.99 & 12.05 & 22.18 & 14.96\\
     %\cline{2-2} \cline{4-11}
     & RelReg & & 35.40 & 11.88 & 22.97 & 21.64 & 31.49 & 8.38 & 20.02 & 17.24\\
     & SegEnc & & 38.53 & 14.99 & 24.98 & 26.26 & 36.62 & 11.77 & 22.99 & 23.26\\
     & \multicolumn{1}{c|}{GPT-3} &  & 42.34 & 16.71 & 29.12 & 34.08 & 39.45 & 13.78 & 26.72 & 31.16\\
     %\cline{2-2} \cline{4-11}
    \hline
    %\cline{2-11}
    %\hline
   \multirow{3}{*}{Zero-shot} & BART & Pipeline & 40.85 & 16.99 & 27.63 & 30.38 & 37.28 & 13.16 & 24.45 & 29.36\\
    %\cline{2-2} \cline{4-11}
    
    %\cline{2-11}
      
   & GPT-3 & Pipeline & 44.49 & 18.51 & 31.21 & \textbf{40.12} & 42.29 & 16.02 & 29.33 & \textbf{37.68}\\
     & \demph{GPT-3} & \demph{Pipeline (Oracle)} & \demph{47.27} & \demph{20.74} & \demph{33.98} & \demph{42.65} & \demph{45.45} & \demph{17.89} & \demph{31.27} & \demph{40.29}\\
    %& BART & \multicolumn{1}{c||}{\multirow{2}{*}{Pipeline (Oracle)}} & 42.20 & 18.26 & 29.54 & & 39.83 & 15.01 & 26.41 & \\\cline{2-2} \cline{4-11}
    %& GPT-3 &  & 47.27 & 20.74 & 33.98 & & 45.45 & 17.89 & 31.27 & \\
    \hline
    
    \multirow{2}{*}{\parbox{4.7em}{\centering + Silver Training}} & SegEnc & QFS & 47.09 & 20.05 & 31.99 & 38.64 & 44.35 & 17.47 & \textbf{29.69} & 36.26\\
    %\cline{2-11}
    & BART & Pipeline & 46.14 & 18.92 & 31.37 & 34.17 & 43.00 & 15.95 & 28.66 & 34.55\\
    %\cline{2-11}
    %& BART & Pipeline (Oracle) & 49.51 & 21.69 & 34.24 & & 46.43 & 18.79 & 31.57  \\
    \hline
    
   \multirow{3}{*}{\parbox{4.7em}{\centering + Gold Finetuning}} & SegEnc & QFS & \textbf{48.30} & \textbf{22.45} & \textbf{32.98} & 39.95 & \textbf{45.06} & \textbf{18.45} & 29.43 & 36.71\\
    %\cline{2-11}
    & BART & Pipeline & 46.59 & 20.38 & 32.31 & 37.78 & 44.38 & 17.53 & 29.62 & 35.72\\
    %\cline{2-11}
    & \demph{BART} & \demph{Pipeline (Oracle)}  & \demph{51.11} & \demph{24.23} & \demph{35.92} & \demph{42.28} & \demph{47.82} & \demph{20.23} & \demph{32.20} & \demph{39.61}\\
    \hline
    
%    Direct FT & BART & Pipeline (Oracle) & 50.02 & 23.91 & 35.05 & 47.24 & 19.53 & 31.41 & &\\
%    \hline
%    \hline
  
    \hline
    \end{tabular}
    \caption{ROUGE and BertScore performance of various models on the SumREN benchmark. We explore both query-focused (QFS) and pipeline-based approaches under zero-shot, silver-training and gold-fine-tuning settings. \textit{Pipeline (Oracle)} corresponds to using the gold reported statements as input to the summarization model and is reported for the best setup for each of the zero-shot and fine-tuned models.}
    \label{tab:model_results}
\vspace{-0.75em}
\end{table*}
%---------------------------------------------------------------
Here, we describe our proposed pipeline-based approach along with several strong baselines that we experiment with. 

%\heng{are you going to add more advanced methods? or only have these baselines? if you only have baselines maybe should send this to the resource track}\ken{I agree this paper is more like a resource paper, AAAI regular papers usually involve new methods. }

%Our proposed task requires generating a summary of the reported statements, given a set of news articles and the name of the speaker as input. In this section, we explore various approaches to build systems for the reported speech summarization task. We broadly categorize these into two kinds: (a) Query-Focused summarization (Section \ref{sec:query-focused}) and (b) Pipeline-Based summarization (Section \ref{sec:pipeline-based}). We describe these in detail below.

\label{sec:query-focused}
\subsection{Query-Focused Summarization Baselines}
Our proposed task requires generating a summary of the reported statements, given a set of news articles and the name of the speaker as input. To leverage existing models, our reported-speech summarization task can be approached as query-focused summarization -- by  generating a summary of the given text conditioned upon a query.  Specifically, given the name of the speaker, the corresponding query can be formulated as: \textit{``Summarize what $<$speaker$>$ said.''}. Following this, we explore multiple query-focused summarization approaches, which we describe below.

\begin{itemize}[]
    \item \textbf{GR-SUM}~\cite{wan2008using} uses an unsupervised graph-based extractive method where each source sentence is treated as a node.\footnote{We use the source code from \citet{DBLP:journals/tacl/CMDPControlSum21}.} It uses a random-walk algorithm to rank the input sentences based on the adjacency weights and the topic relevance vectors for each node. 
    \item \textbf{RelReg}~\cite{vig2021exploring} uses a two-step process. First a regression model is used to extract a contiguous span within the input that is relevant to the input query. The extracted context is then passed along with the query to a BART model to generate a summary. Both the regression and BART models are trained on QMSum~\cite{DBLP:conf/naacl/QMSum21}, a query-focused meeting summarization dataset. 
    \item \textbf{SegEnc}~\cite{vig2021exploring} is an end-to-end generative model that first splits the source documents into overlapping text segments. Each of these segments is then concatenated with the input query and independently encoded by a Transformer encoder. The encoded segments are then concatenated into a sequence of vectors and fed into a Transformer decoder to generate the summary. The model is pre-trained on WikiSum dataset \cite{DBLP:conf/iclr/wikisum18} and finetuned on QMSum dataset \cite{zhong2021qmsum}. 
    \item \textbf{GPT-3}: In addition to these baselines, we also explore directly providing the source news articles as input to GPT-3  and using the query as the prompt.
\end{itemize}

\begin{comment}
\subsubsection{GR-SUM} ~\cite{wan2008using} uses an unsupervised graph-based extractive method where each source sentence is treated as a node. %The adjacency weight between a pair of nodes uses the cosine similarity between their TF-IDF vectors. 
%This method computes a top-relevance score for each node based on the topic-level similarity to the input query. 
It uses a random-walk algorithm to rank the input sentences based on the adjacency weights and the topic relevance vectors for each node. %In our experiments, we return the top $3$ sentences according to the empirical performance on the development set. 

%It then uses random-walk algorithm similar to PageRank to rank the importance

\subsubsection{RelReg} ~\cite{vig2021exploring} uses a two-step process. % for query-focused summarization. 
It first uses a regression model to extract a contiguous span within the input that is relevant to the input query. The extracted context is then passed along with the query to a BART model to generate a summary. 
Both the regression and BART models are trained on QMSum~\cite{DBLP:conf/naacl/QMSum21} query-focused dialog summarization dataset. 

\subsubsection{SegEnc} ~\cite{vig2021exploring} is an end-to-end generative model that first splits the source documents into overlapping text segments. 
Each of these segments is then concatenated with the input query and independently encoded by a Transformer encoder. The encoded segments are then concatenated into a sequence of vectors and fed into a Transformer decoder to generate the summary. This model is pre-trained on WikiSum dataset \cite{DBLP:conf/iclr/wikisum18} and finetuned on QMSum dataset \cite{zhong2021qmsum}. 

\subsubsection{GPT-3} In addition to these baselines, we also explore directly providing the source news articles as input to GPT-3  and using the query as the prompt.
\end{comment}
%\heba{Revanth: Please make sure that what I wrote here is an accurate description of the GPT-3 baseline.} 
%In our Segment Encoder (SEGENC) model, the source document is split into fixed-length overlapping1 segments, each of which is separately appended to the query and encoded us- ing a standard Transformer model.
%Similar to FiD, these encodings are then concatenated into a sin- gle embedding sequence and passed to a decoder model that generates the summary.
%--------------------------------------------------------------
\subsection{Pipeline-based Summarization Framework}
\label{sec:pipeline-based}
We utilitize a pipeline-based approach for summarizing reported speech. 
%Similar to our annotation task, 
The proposed pipeline involves three main steps; (1) extracting reported statements and their speakers from the given set of news articles, (2) grouping statements together that come from the same speaker, and (3) generating a summary for each group of reported statements.

\subsubsection{Reported Speech Extraction:}
\label{sec:reported_extraction}
Given a collection of news articles and a speaker, we aim to identify all reported statements along with the corresponding speakers. To this end, we build a span-tagging system that leverages a Transformer-based encoder to identify the spans of statements and the corresponding speaker. The model is trained using the PolNeAR corpus \cite{newell2018attribution} which 
provides annotated triples of \textit{source} (i.e. speaker), \textit{cue} (i.e. words that indicate the presence of attribution), and \textit{content} (i.e. the statements made by the speaker) for statements made in the news. 
%\heba{Thanks for the explanation Ken. //Revanth: I am not sure I follow the next sentence. How is it different from the sentences before it? What exactly provides richer supervision signals?} \ken{In reported speech extraction, we do not need to extract the cues, but during model training, we also train the model to extract the cues to provide richer supervision signals about the words that indicate the presence of attribution. I think we can move the next sentence to the implementation details section of the Appendix to reduce space. }
%We also train a span tagging model to predict the spans of cues to provide richer supervision signals about the words that indicate the presence of attribution.
%\footnote{We assume each paragraph contains at most three triples of (statement, cue, speaker). The total number of BIO tags is $19$.}. 

Given an input paragraph of length $T$, we use a BERT encoder to learn the representation $H \in R^{TXD}$ -- of hidden dimension $D$ -- for the input sequence. We then add a binary classification head to identify whether or not the input paragraph contains a reported statement and a $BIO$ sequence labeling head to identify the spans of the statement and the speaker. 
%\ken{the semi-colons in this sentence are weird}
The binary classification $y^{cls}$ and the token label $Y^{span}_i\in R^K$ probabilities are calculated as follows:
%Ken: I use the align environment since it provide a equation number and reviewers can refer to it easily
\begin{align}
   y^{cls}  &= \sigma(w^{cls} \cdot H_{CLS} + b^{cls}) \\
   Y^{span}_i  &= \text{softmax}(W^{sp} H_i + b^{sp})
\end{align}
where $w^{cls}\in R^D$ and $W^{sp}\in R^{K\times D}$ are the weights, $b^{cls}$ and $b^{sp}$ are the bias terms, $K$ is the total number of $BIO$ tags, $H_{CLS}$ and $H_i$ denote the representation of the $CLS$ token and the $i$-th token respectively. 

Finally, the model is trained with a multi-task learning objective by using a joint loss that performs a weighted sum of the classification -- binary cross entropy (BCE) -- and the sequence labeling head -- Cross Entropy (CE) -- losses.
\begin{align}
    L = \alpha \cdot \textbf{} BCE(y^{cls}, \hat{y}^{cls}) + \beta \cdot  CE(Y^{sp}, \hat{Y}^{sp})
\end{align}
where $y^{cls}$ and $\hat{y}^{cls}$ correspond to the predicted and ground-truth classification label respectively, $Y^{sp}$ and $\hat{Y}^{sp}$ denote the predcited and ground-truth token labels respectively, $\alpha$ and $\beta$ are tunable hyper-parameters.\footnote{In our experiments, we set $\alpha$ to $1$ and $\beta$  to $0.4$.} 
%the weight associated to each loss
%\heba{Please describe every symbol listed in the equations even if obvious, such as weight, bias, predicted label, etc.}
%\revanth{Added descriptions for weight, bias and predicted labels}
\subsubsection{Speaker Co-reference Resolution:}
In order to group the statements by the speaker, we need to perform co-reference resolution since speakers can be referred to by different nominal (e.g., Biden, Joe Biden, Joe R. Biden) and pronominal (e.g., He) mentions. To achieve this, we utilize an existing information extraction system \cite{li2020gaia}, which leverages co-reference resolution from \citet{lai2022end}. As we show later, using co-reference resolution considerably increases the coverage of reported statements by a given speaker.
%---------------------------------------------------------------
\subsubsection{Summary Generation:}
\label{sec:summarizing}
Given a set of reported statements for a speaker, we aim to generate a concise summary of the statements.
The summary generation process for the extracted reported statements of a given speaker is akin to single-document summarization. The reported statements are concatenated before getting passed as input to a BART \cite{lewis2020bart} model. The summarization model, trained on CNN-DailyMail \cite{hermann2015teaching}, is first used in a zero-shot setting. This model then undergoes silver-training and gold-finetuning, the details of which are provided in Section \ref{sec:train_setup}.
%\heba{Revanth: I think we need to explain the different approaches for fine-tuning on gold and/or silver data versus no fine-tuning.} 
%Also, I re-arranged the rows in Table 3 to clearly show which ones are off-the-shelf versus using our proposed framework.

%, which contains bullet point summaries of news articles from the CNN and DailyMail publishers.






%\begin{table}[!htb]
%\footnotesize
%    \centering
%    \begin{tabular}{p{8em}|c|c}
%    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Approach}}} & \textbf{Dev} & \textbf{Test} \\
    %\cline{2-3}
%     & \textbf{R-1/R-2/R-L} & \textbf{R-1/R-2/R-L} \\
%    \hline
%    Silver Train + \newline Gold Finetune & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{51.11}/24.23/35.92}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{47.82}/\textbf{20.23}/\textbf{32.20}}}\\
 %   \hline
 %   Direct Gold \newline Finetune & \multicolumn{1}{c|}{\multirow{2}{*}{50.02/23.91/35.05}} & \multicolumn{1}{c}{\multirow{2}{*}{47.24/19.53/31.41}}\\
 %   \hline
 %   Parameter-efficient Gold Finetune & \multicolumn{1}{c|}{\multirow{2}{*}{50.71/\textbf{24.64}/\textbf{36.09}}} & \multicolumn{1}{c}{\multirow{2}{*}{47.75/\textbf{20.23}/31.84}}\\
 %   \hline
 %   \end{tabular}
  %  \caption{Table showing benefit of using silver standard training data. The different approaches compared for BART when used for summarization with oracle reported statements}
 %   \label{tab:silver_training_benefit}
%\end{table}


==> camera_ready_sections/related_work.tex <==
Our work draws from multiple related research veins
as itemized in this section.
%including abstractive news summarization, query-focused summarization, and author attribution in news. 
\paragraph{News Summarization:} Summarizing news articles has been extensively studied in existing literature with multiple existing datasets. Single document summarization datasets include CNN/Daily Mail~\cite{hermann2015teaching},  News Room corpus \cite{grusky2018newsroom} and the XSum dataset~\cite{narayan2018don}. \citet{fabbri2019multi} introduce a large-scale dataset, Multi-News, to extend news summarization to a multi-document setting.  Timeline summarization \cite{steen2019abstractive, li2021timeline} adds a temporal aspect to news summarization by generating a sequence of major news events with their key dates. % from a large collection of related news from multiple perspectives.
Another line of work lies around news headline generation \cite{banko2000headline}, which involves generating representative headlines for a given news story, explored in both single- \cite{hayashi2018headline} and multi-document settings \cite{gu2020generating}. However, these datasets all largely focus on summarizing the details of events and neglect the reported speech related to these events.

% Heba: Commenting because this is mentioned several times before.
%However, current tasks around news summarization consider summarizing the event in the news story. Instead, our task focuses on summarizing the statements that people have made in news articles about these events. This aims to capture the reactions to such news events.

%\paragraph{Other summarization tasks:}
\paragraph{Query-Focused Summarization:}
%\revanth{Finished re-writing the two paragraphs below, please take a look.}
Query-focused summarization (QFS) aims to produce a summary that answers a specific query about the source document(s). Conceptually, reported speech summarization corresponds to the query, {\em ``What did X say about Y?"}.
Prior work builds large-scale QFS datasets by obtaining reference summaries by scraping them from the web or using pseudo-heuristics. For example,  WikiSum~\cite{DBLP:conf/iclr/wikisum18} and AQuaMuSe~\cite{DBLP:journals/corr/aquamuse2020} directly extract paragraphs from Wikipedia articles as reference summaries. On the other hand, manually annotated QFS datasets are small -- DUC 2006 and 2007 \cite{dang2005overview} contain up to only 50 examples. QMSum~\cite{zhong2021qmsum} focuses on summarizing meeting dialogue transcripts and is most similar to our work. However, QMSum transcripts contain a considerable amount of informal conversations and do not contain focused informative content like the reported statements in \textsc{SumREN}. 

Since QFS datasets usually come with only source-summary pairs, most prior work either use end-to-end approaches  \cite{vig2021exploring,DBLP:journals/tacl/LatenQuery22} or follow a two-step extract-then-abstract framework \cite{DBLP:conf/acl/XuL20, vig2021exploring}, with the extractor trained to identify text spans that are similar to the reference summary in terms of ROUGE scores. Conversely, \textsc{SumREN} additionally provides the corresponding relevant content, reported statements in this case, that was used to annotate the summaries. Thereby, our proposed pipeline-based approach can leverage this to build and evaluate an extractive component that is independent of the reference summary, while still ensuring the generated summary has high input fidelity in terms of factual consistency.
%QMSum~\cite{zhong2021qmsum}, which focuses on summarizing meeting dialogue transcripts is most similar to our work. However, the transcripts in QMSum contain considerable amount of informal conversations and do not contain focused informative content like the reported statements in \textsc{SumREN}. 

%Prior literature propose various QFS datasets. The WikiSum~\cite{DBLP:conf/iclr/wikisum18} dataset treats the title of a Wikipedia article as the query. The documents cited by the article are acted as the input and the first paragraph of the article is used as the reference summary. AQuaMuSe~\cite{DBLP:journals/corr/aquamuse2020} employs user queries in search engines as the input query and extract paragraphs from Wikipedia articles as the reference summaries. The Debatepedia dataset~\cite{DBLP:conf/acl/debate17} crawls the questions, argument articles, and summaries from the Debatepedia database as the queries, source documents, and ground-truth summaries respectively. 
%
%QMSum~\cite{zhong2021qmsum} focuses on summarizing meeting dialogues and crowd-sourced queries and summaries for meeting transcripts. The DUC 2006 and 2007 datasets~\cite{dang2005overview} collect clusters of news articles and ask humans to annotate the questions and the corresponding summaries. The questions in the DUC datasets are mainly related to the events described by the news. %On the contrary, our proposed task aims to summarize statements said by a specific person in news articles. 

%Most of the previous literature on QFS relies on extractive summarization ~\cite{DBLP:conf/emnlp/XuL20,DBLP:conf/sigir/CTSumWanZ14,wan2008using,DBLP:conf/ijcai/WanX09}. Recently, \citet{vig2021exploring} proposed a generative model that separately encodes each source document fragment by a Transformer encoder and then generates the output summary by a Transformer decoder.  ~\citet{DBLP:conf/acl/XuL20, vig2021exploring} follows a two-step pipeline that first extracts relevant spans from the source and then synthesizes them into a summary. In these methods, the extractor is trained to extract the text spans that are similar to the reference summary in terms of ROUGE scores. 
 %Similarity, our method also follows an extract-then-abstract pipeline.  In contrast, our extractor is trained to extract reported statements on a news attribution dataset.% and is independent of the reference summary.
 %Similarly, we rely on a two-step pipeline to first extract the reported statements before summarizing them. 
 %In contrast to QFS, the extraction step is independent of the reference summary.
 %\heba{Revanth:Please highlight the difference between our extractor and QFS}

%Both the DUC datasets and our \textsc{SumREN} dataset contain multiple reference summaries for each sample. However, each of these DUC datasets only has around 50 clusters of source articles while \textsc{SumREN} consists of \ken{XXXX} clusters of articles.  
%\ken{I did not emphasis the multi-reference here since DUC datasets also contain multi-reference. }
%\ken{It may be better to only discuss query-focused summarization in the related work since other tasks like scientific document summarization and government report summarization are less related to our task. }

%Some other datasets crawl questions and documents from StackExchange~\cite{DBLP:conf/naacl/AnswerSum22} and Wikihow~\cite{DBLP:conf/aaai/wikihowsum20} and annotate reference summaries. 


% highlight the differences

% query types
% multireference
% annotation vs craw
%---------------------------------------------------------------
\paragraph{Attribution in News:}  Attribution has been well-studied with multiple available datasets. \citet{elson2010automatic, zhang2021directquote} study attribution of direct quotations along with their speakers. 
%\heba{I don't think this sentence is clear. What does ``with their sources'' mean here} 
\citet{pareti2012database, pareti2013automatically} extend this notion by including indirect quotations and create the PARC3 corpus. %The corpus includes annotations for the source (i.e. speaker) and content spans, as well as the cues (i.e. words that indicate the presence of attribution).
More recently, PolNeAR \cite{newell2018attribution} was created to improve upon PARC3 by doubling the recall and improving inter-annotator agreement. However, all of these lines of work solely deal with identifying attribution and do not aggregate extracted statements from specific speakers to help with a downstream task. More direct uses of quotations in news include opinion mining \cite{balahur2009opinion} and sentiment analysis \cite{balahur2013sentiment}.  In contrast, our proposed task involves attribution to identify reported statements in news articles, which are then aggregated and summarized to convey the reactions to events in news. 
%\heng{I summarized a lot of more work in http://blender.cs.illinois.edu/KDD22\_tutorial\_slides\_Heng.pptx  Please add more of these related papers}
%Attribution has been actively used in various NLP tasks. Datasets on discourse parsing and analysis \cite{prasad2008penn, wolf2005representing} include the use of attribution phenomena. However, these corpora are not specific to attribution and do not consider key elements of attributions, such as the source. 
%A more direct use of quotations in news has been for opinion mining \cite{balahur2009opinion} to discover opinions and sentiment analysis \cite{balahur2013sentiment} to evaluate the author's mood.  In contrast, our proposed task involves attribution to identify reported statements in news articles, which are then summarized to convey the reactions to events in news.
%---------------------------------------------------------------
